Combining Stochastic Defenses to Resist Gradient Inversion: An Ablation Study

Gradient Inversion (GI) attacks are a ubiquitous threat in Federated Learning (FL) as they exploit gradient leakage to reconstruct supposedly private training data. Common defense mechanisms such as Differential Privacy (DP) or stochastic Privacy Modules (PMs) introduce randomness during gradient computation to prevent such attacks. However, we pose that if an attacker effectively mimics a client's stochastic gradient computation, the attacker can circumvent the defense and reconstruct clients' private training data. This paper introduces several targeted GI attacks that leverage this principle to bypass common defense mechanisms. As a result, we demonstrate that no individual defense provides sufficient privacy protection. To address this issue, we propose to combine multiple defenses. We conduct an extensive ablation study to evaluate the influence of various combinations of defenses on privacy protection and model utility. We observe that only the combination of DP and a stochastic PM was sufficient to decrease the Attack Success Rate (ASR) from 100% to 0%, thus preserving privacy. Moreover, we found that this combination of defenses consistently achieves the best trade-off between privacy and model utility.

==> tables/Ablation2.tex <==
\begin{table*}[t]
\centering
\caption{
Model utility and privacy metrics for an ablation study using different combinations of defense mechanisms in the \ac{CNN} on the MNIST dataset. 
% The training gradients are attacked with \ac{CDIA} (\cf \autoref{alg:CDIA}).
We consider Dropout (DO), \acf{DP}, \acf{GP} and a \acf{PM} as defense.
\cmark and \textcolor[HTML]{cfcfcf}{\xmark} indicate, whether a defense mechanism was used or not.
P and C indicate whether \ac{PRECODE} or \ac{CVB} was used, respectively.
Arrows indicate direction of improvement from the viewpoint of a defending client.
Bold and italic formatting highlight best and worst results, respectively.
}
\label{tab:results_xcomb_ablation_mnist}
% \resizebox{0.9\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
 & DO & \ac{DP} & \ac{GP} & PM & \ac{SSIM} $\downarrow$ & \ac{ASR} [\%] $\downarrow$ & Accuracy [\%] $\uparrow$ \\
\midrule
\multirow[c]{24}{*}{\rotatebox{90}{MNIST}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} 0.95 ($\pm$0.06) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.10 ($\pm$0.04) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} 0.95 ($\pm$0.07) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.33 ($\pm$0.02) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{DC3B2C}} \color[HTML]{F1F1F1} 0.88 ($\pm$0.09) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.15 ($\pm$0.05) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} 0.95 ($\pm$0.04) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.00 ($\pm$0.09) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & P & {\cellcolor[HTML]{C62027}} \color[HTML]{F1F1F1} 0.93 ($\pm$0.09) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.41 ($\pm$0.04) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & C & {\cellcolor[HTML]{E75337}} \color[HTML]{F1F1F1} 0.84 ($\pm$0.08) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.06 ($\pm$0.05) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{C62027}} \color[HTML]{F1F1F1} 0.93 ($\pm$0.06) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.06 ($\pm$0.00) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{FBFDBA}} \color[HTML]{000000} 0.49 ($\pm$0.12) & {\cellcolor[HTML]{FFFDBC}} \color[HTML]{000000} 50.78 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} \itshape 98.19 ($\pm$0.03) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{36A657}} \color[HTML]{F1F1F1} 0.14 ($\pm$0.05) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.18 ($\pm$0.00) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} 0.95 ($\pm$0.05) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 98.97 ($\pm$0.05) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & P & {\cellcolor[HTML]{FFFEBE}} \color[HTML]{000000} 0.50 ($\pm$0.13) & {\cellcolor[HTML]{FFF0A6}} \color[HTML]{000000} 54.69 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.22 ($\pm$0.14) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & C & {\cellcolor[HTML]{36A657}} \color[HTML]{F1F1F1} 0.14 ($\pm$0.04) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 99.19 ($\pm$0.05) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 0.97 ($\pm$0.02) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.12 ($\pm$0.03) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 0.97 ($\pm$0.04) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.41 ($\pm$0.02) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{D22B27}} \color[HTML]{F1F1F1} 0.91 ($\pm$0.06) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.09 ($\pm$0.08) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} \itshape 0.97 ($\pm$0.02) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 98.95 ($\pm$0.06) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & P & {\cellcolor[HTML]{B91326}} \color[HTML]{F1F1F1} 0.96 ($\pm$0.06) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.24 ($\pm$0.03) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & C & {\cellcolor[HTML]{E54E35}} \color[HTML]{F1F1F1} 0.85 ($\pm$0.09) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.05 ($\pm$0.03) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{FEEC9F}} \color[HTML]{000000} 0.56 ($\pm$0.14) & {\cellcolor[HTML]{FDB163}} \color[HTML]{000000} 69.53 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.06 ($\pm$0.05) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{D9EF8B}} \color[HTML]{000000} 0.40 ($\pm$0.20) & {\cellcolor[HTML]{D3EC87}} \color[HTML]{000000} 39.06 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.28 ($\pm$0.00) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{279F53}} \color[HTML]{F1F1F1} \bfseries 0.12 ($\pm$0.06) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.12 ($\pm$0.01) \\
 & \cmark & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{FEEC9F}} \color[HTML]{000000} 0.56 ($\pm$0.14) & {\cellcolor[HTML]{FBA05B}} \color[HTML]{000000} 71.88 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 98.95 ($\pm$0.04) \\
 & \cmark & \cmark & \cmark & P & {\cellcolor[HTML]{C9E881}} \color[HTML]{000000} 0.37 ($\pm$0.19) & {\cellcolor[HTML]{93D168}} \color[HTML]{000000} 27.34 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 98.23 ($\pm$0.03) \\
 & \cmark & \cmark & \cmark & C & {\cellcolor[HTML]{279F53}} \color[HTML]{F1F1F1} \bfseries 0.12 ($\pm$0.05) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 99.15 ($\pm$0.06) \\
\bottomrule
\end{tabular} %
% }
\end{table*}

\begin{table*}[th]
\centering
\caption{
Model utility and privacy metrics for an ablation study using different combinations of defense mechanisms in the \ac{CNN} on the CIFAR-10 dataset. 
% The training gradients are attacked with \ac{CDIA} (\cf \autoref{alg:CDIA}).
We consider Dropout (DO), \acf{DP}, \acf{GP} and a \acf{PM} as defense.
\cmark and \color[HTML]{cfcfcf} \xmark~indicate, whether a defense mechanism was used or not.
P and C indicate whether \ac{PRECODE} or \ac{CVB} was used, respectively.
% Details on the used parameters for each defense mechanism can be found in \autoref{sec:setup_xcomb_ablation}. 
Arrows indicate direction of improvement from the viewpoint of a defending client.
Bold and italic formatting highlight best and worst results, respectively.
}
\label{tab:results_xcomb_ablation_cifar}
% \resizebox{0.95\linewidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
 & DO & \ac{DP} & \ac{GP} & PM & \ac{SSIM} $\downarrow$ & \ac{ASR} [\%] $\downarrow$ & Accuracy [\%] $\uparrow$ \\
\midrule
\multirow[c]{24}{*}{\rotatebox{90}{CIFAR-10}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} 0.87 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} 96.88 & {\cellcolor[HTML]{17934E}} \color[HTML]{F1F1F1} 62.53 ($\pm$0.16) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{DC3B2C}} \color[HTML]{F1F1F1} 0.88 ($\pm$0.07) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} 59.48 ($\pm$0.23) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{FBA05B}} \color[HTML]{000000} 0.72 ($\pm$0.13) & {\cellcolor[HTML]{C21C27}} \color[HTML]{F1F1F1} 93.75 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 67.19 ($\pm$0.64) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{E24731}} \color[HTML]{F1F1F1} 0.86 ($\pm$0.09) & {\cellcolor[HTML]{AB0626}} \color[HTML]{F1F1F1} 98.44 & {\cellcolor[HTML]{17934E}} \color[HTML]{F1F1F1} 62.53 ($\pm$0.34) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & P & {\cellcolor[HTML]{E24731}} \color[HTML]{F1F1F1} 0.86 ($\pm$0.10) & {\cellcolor[HTML]{AB0626}} \color[HTML]{F1F1F1} 98.44 & {\cellcolor[HTML]{39A758}} \color[HTML]{F1F1F1} 59.53 ($\pm$0.11) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \cmark & C & {\cellcolor[HTML]{FDC372}} \color[HTML]{000000} 0.66 ($\pm$0.09) & {\cellcolor[HTML]{C62027}} \color[HTML]{F1F1F1} 92.97 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 67.34 ($\pm$0.28) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{EB5A3A}} \color[HTML]{F1F1F1} 0.83 ($\pm$0.11) & {\cellcolor[HTML]{AF0926}} \color[HTML]{F1F1F1} 97.66 & {\cellcolor[HTML]{18954F}} \color[HTML]{F1F1F1} 62.31 ($\pm$0.00) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{D9EF8B}} \color[HTML]{000000} 0.40 ($\pm$0.14) & {\cellcolor[HTML]{89CC67}} \color[HTML]{000000} 25.78 & {\cellcolor[HTML]{57B65F}} \color[HTML]{F1F1F1} 57.39 ($\pm$0.26) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} \bfseries 0.04 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{08773F}} \color[HTML]{F1F1F1} 65.86 ($\pm$0.25) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{F16640}} \color[HTML]{F1F1F1} 0.81 ($\pm$0.10) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} 96.88 & {\cellcolor[HTML]{2AA054}} \color[HTML]{F1F1F1} 60.72 ($\pm$0.51) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & P & {\cellcolor[HTML]{BFE47A}} \color[HTML]{000000} 0.35 ($\pm$0.14) & {\cellcolor[HTML]{4BB05C}} \color[HTML]{F1F1F1} 16.41 & {\cellcolor[HTML]{66BD63}} \color[HTML]{F1F1F1} \itshape 56.26 ($\pm$0.01) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \cmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} \bfseries 0.04 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} 65.45 ($\pm$1.04) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{D22B27}} \color[HTML]{F1F1F1} \itshape 0.91 ($\pm$0.05) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{0F8446}} \color[HTML]{F1F1F1} 64.36 ($\pm$0.12) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{DA362A}} \color[HTML]{F1F1F1} 0.89 ($\pm$0.07) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{36A657}} \color[HTML]{F1F1F1} 59.77 ($\pm$0.16) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{F88C51}} \color[HTML]{F1F1F1} 0.75 ($\pm$0.08) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 67.80 ($\pm$0.41) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{DC3B2C}} \color[HTML]{F1F1F1} 0.88 ($\pm$0.05) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{17934E}} \color[HTML]{F1F1F1} 62.43 ($\pm$0.24) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & P & {\cellcolor[HTML]{E0422F}} \color[HTML]{F1F1F1} 0.87 ($\pm$0.07) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{36A657}} \color[HTML]{F1F1F1} 59.83 ($\pm$0.34) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \cmark & C & {\cellcolor[HTML]{FDBD6D}} \color[HTML]{000000} 0.67 ($\pm$0.11) & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} 95.31 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 67.68 ($\pm$0.48) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{C9E881}} \color[HTML]{000000} 0.37 ($\pm$0.14) & {\cellcolor[HTML]{60BA62}} \color[HTML]{F1F1F1} 19.53 & {\cellcolor[HTML]{148E4B}} \color[HTML]{F1F1F1} 63.21 ($\pm$0.27) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & P & {\cellcolor[HTML]{ABDB6D}} \color[HTML]{000000} 0.31 ($\pm$0.17) & {\cellcolor[HTML]{3CA959}} \color[HTML]{F1F1F1} 14.84 & {\cellcolor[HTML]{57B65F}} \color[HTML]{F1F1F1} 57.32 ($\pm$0.19) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} \bfseries 0.04 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{07753E}} \color[HTML]{F1F1F1} 66.00 ($\pm$0.42) \\
 & \cmark & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{C9E881}} \color[HTML]{000000} 0.37 ($\pm$0.13) & {\cellcolor[HTML]{4BB05C}} \color[HTML]{F1F1F1} 16.41 & {\cellcolor[HTML]{1E9A51}} \color[HTML]{F1F1F1} 61.51 ($\pm$0.14) \\
 & \cmark & \cmark & \cmark & P & {\cellcolor[HTML]{87CB67}} \color[HTML]{000000} 0.25 ($\pm$0.17) & {\cellcolor[HTML]{108647}} \color[HTML]{F1F1F1} 6.25 & {\cellcolor[HTML]{66BD63}} \color[HTML]{F1F1F1} \itshape 56.26 ($\pm$0.01) \\
 & \cmark & \cmark & \cmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} \bfseries 0.04 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} 65.38 ($\pm$1.01) \\
\bottomrule
\end{tabular} %
% }
\end{table*}


==> tables/Datasets.tex <==
\begin{table*}[h!]
\centering
\caption{
Model utility and privacy metrics for an ablation study using different combinations of defense mechanisms in the \ac{CNN} on different MedMNIST datasets. 
% The training gradients are attacked with \ac{CDIA} (\cf \autoref{alg:CDIA}).
We consider Dropout (DO), \acf{DP}, \acf{GP} and a \acf{PM} as defense.
\cmark and \textcolor[HTML]{cfcfcf}{\xmark} indicate, whether a defense mechanism was used or not.
P and C indicate whether \ac{PRECODE} or \ac{CVB} was used, respectively.
% Details on the used parameters for each defense mechanism can be found in \autoref{sec:setup_xcomb_data}. 
Arrows indicate direction of improvement from the viewpoint of a defending client.
Bold and italic formatting highlight best and worst results, respectively.
}
\label{tab:results_xcomb_datasets}
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
& DO & \ac{DP} & \ac{GP} & PM & \ac{SSIM} $\downarrow$ & \ac{ASR} [\%] $\downarrow$ & Accuracy [\%] $\uparrow$ \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{Blood}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{DC3B2C}} \color[HTML]{F1F1F1} 0.88 ($\pm$0.11) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} 96.88 & {\cellcolor[HTML]{05713C}} \color[HTML]{F1F1F1} 90.67 ($\pm$1.03) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{F57245}} \color[HTML]{F1F1F1} 0.79 ($\pm$0.10) & {\cellcolor[HTML]{C01A27}} \color[HTML]{F1F1F1} 94.53 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 92.42 ($\pm$0.29) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{E54E35}} \color[HTML]{F1F1F1} 0.85 ($\pm$0.12) & {\cellcolor[HTML]{C01A27}} \color[HTML]{F1F1F1} 94.53 & {\cellcolor[HTML]{06733D}} \color[HTML]{F1F1F1} \itshape 90.18 ($\pm$0.67) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0F8446}} \color[HTML]{F1F1F1} \bfseries 0.06 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 92.15 ($\pm$0.23) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{CC2627}} \color[HTML]{F1F1F1} \itshape 0.92 ($\pm$0.04) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{06733D}} \color[HTML]{F1F1F1} 90.48 ($\pm$0.73) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0F8446}} \color[HTML]{F1F1F1} \bfseries 0.06 ($\pm$0.03) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 92.36 ($\pm$0.56) \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{Derma}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{E24731}} \color[HTML]{F1F1F1} 0.86 ($\pm$0.14) & {\cellcolor[HTML]{B91326}} \color[HTML]{F1F1F1} 96.09 & {\cellcolor[HTML]{026C39}} \color[HTML]{F1F1F1} 74.80 ($\pm$0.15) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{FDC776}} \color[HTML]{000000} 0.65 ($\pm$0.20) & {\cellcolor[HTML]{EC5C3B}} \color[HTML]{F1F1F1} 82.81 & {\cellcolor[HTML]{016A38}} \color[HTML]{F1F1F1} 75.00 ($\pm$0.71) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{F57245}} \color[HTML]{F1F1F1} 0.79 ($\pm$0.15) & {\cellcolor[HTML]{C21C27}} \color[HTML]{F1F1F1} 93.75 & {\cellcolor[HTML]{05713C}} \color[HTML]{F1F1F1} 73.87 ($\pm$0.57) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} 0.04 ($\pm$0.03) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{06733D}} \color[HTML]{F1F1F1} \itshape 73.69 ($\pm$1.17) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{CC2627}} \color[HTML]{F1F1F1} \itshape 0.92 ($\pm$0.09) & {\cellcolor[HTML]{AB0626}} \color[HTML]{F1F1F1} \itshape 98.44 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 75.36 ($\pm$0.08) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{07753E}} \color[HTML]{F1F1F1} \bfseries 0.03 ($\pm$0.03) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{06733D}} \color[HTML]{F1F1F1} 73.74 ($\pm$0.13) \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{Pneumonia}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} \itshape 0.95 ($\pm$0.04) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{036E3A}} \color[HTML]{F1F1F1} 86.37 ($\pm$0.09) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{FDC372}} \color[HTML]{000000} 0.66 ($\pm$0.09) & {\cellcolor[HTML]{C01A27}} \color[HTML]{F1F1F1} 94.53 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 87.35 ($\pm$1.22) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{CC2627}} \color[HTML]{F1F1F1} 0.92 ($\pm$0.07) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{05713C}} \color[HTML]{F1F1F1} \itshape 85.83 ($\pm$0.91) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{0A7B41}} \color[HTML]{F1F1F1} 0.04 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{016A38}} \color[HTML]{F1F1F1} 86.81 ($\pm$0.75) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{BD1726}} \color[HTML]{F1F1F1} \itshape 0.95 ($\pm$0.07) & {\cellcolor[HTML]{A70226}} \color[HTML]{F1F1F1} 99.22 & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 86.05 ($\pm$0.68) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{07753E}} \color[HTML]{F1F1F1} \bfseries 0.03 ($\pm$0.02) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 87.08 ($\pm$0.77) \\
\midrule
\multirow[c]{6}{*}{\rotatebox{90}{Retina}} & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{E24731}} \color[HTML]{F1F1F1} 0.86 ($\pm$0.13) & {\cellcolor[HTML]{B30D26}} \color[HTML]{F1F1F1} 96.88 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 55.11 ($\pm$0.40) \\
 & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{FEDA86}} \color[HTML]{000000} 0.61 ($\pm$0.15) & {\cellcolor[HTML]{E44C34}} \color[HTML]{F1F1F1} 85.16 & {\cellcolor[HTML]{04703B}} \color[HTML]{F1F1F1} 54.38 ($\pm$1.27) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{F67F4B}} \color[HTML]{F1F1F1} 0.77 ($\pm$0.14) & {\cellcolor[HTML]{C01A27}} \color[HTML]{F1F1F1} 94.53 & {\cellcolor[HTML]{08773F}} \color[HTML]{F1F1F1} 53.53 ($\pm$1.00) \\
 & \color[HTML]{cfcfcf} \xmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{07753E}} \color[HTML]{F1F1F1} 0.03 ($\pm$0.01) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{138C4A}} \color[HTML]{F1F1F1} 51.76 ($\pm$0.31) \\
 & \cmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & \color[HTML]{cfcfcf} \xmark & {\cellcolor[HTML]{D22B27}} \color[HTML]{F1F1F1} \itshape 0.91 ($\pm$0.06) & {\cellcolor[HTML]{A50026}} \color[HTML]{F1F1F1} \itshape 100 & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} 55.03 ($\pm$1.21) \\
 & \cmark & \cmark & \color[HTML]{cfcfcf} \xmark & C & {\cellcolor[HTML]{05713C}} \color[HTML]{F1F1F1} \bfseries 0.02 ($\pm$0.01) & {\cellcolor[HTML]{006837}} \color[HTML]{F1F1F1} \bfseries 0 & {\cellcolor[HTML]{148E4B}} \color[HTML]{F1F1F1} \itshape 51.41 ($\pm$0.15) \\
\bottomrule
\end{tabular}
\end{table*}

